Precision and Recall for Range-Based Anomaly Detection

Classical anomaly detection is principally concerned with point-based anomalies, anomalies that occur at a single data point. In this paper, we present a new mathematical model to express range-based anomalies, anomalies that occur over a range (or period) of time.

==> motivation.tex <==
\section{Design Goals} \label{sec:motivation}

\begin{figure*}[!ht]
\begin{center}
\subfloat[Precision = 0.6, Recall = 0.5]{
\includegraphics[width=0.3\textwidth]{figures/points2.png}
\label{fig:points}
}
\subfloat[Precision = ?, Recall = ?]{
\includegraphics[width=0.5\textwidth]{figures/intervals2.png}
\label{fig:intervals}
}
\caption{Point-based Anomalies vs. Range-based Anomalies}
\label{fig:anomalies}
\end{center}
\end{figure*}

%The goal of this work is to design a mathematical model which can be used to evaluate, rank, and compare results of anomaly detection (AD) algorithms. We particularly focus on algorithms that target range-based anomalies over sequential data \cite{ad-survey}  e.g., time-series. Thus, each anomaly can span a contiguous interval of time. To contrast with ``point-based anomalies", we call these ``range-based anomalies".
%
%An AD algorithm is a form of pattern recognition and binary classification algorithm in that it recognizes certain patterns in its input and classifies them as either normal or anomalous. For this general class of algorithms, relevance measures of Precision and Recall are widely used for evaluating the accuracy of the result . Recall measures what fraction of the real anomaly set ($R$) an algorithm was able to predict correctly, whereas Precision measures what fraction of the predicted anomaly set ($P$) coincides with $R$. 
Traditionally, recall and precision are defined for sets of points, where each point in a set is treated as independent and identical in terms of importance. Therefore, both measures are purely based on relative set sizes (see Figure \ref{fig:points} for an example). This is good enough for AD algorithms designed for detecting  point-based anomalies in a given set. Time-series AD algorithms, on the other hand, work with sequences of time intervals (see Figure \ref{fig:intervals} for an example). As a result, the traditional model is not expressive enough to capture various nuances that may appear in the results of these algorithms.

A significant portion of these nuances are due to {\em partial overlaps}. In the point-based case, a predicted anomaly point $P_i$ is either a member of the set of real anomalies (a TP in Figure \ref{fig:points}) or not (an FP in Figure \ref{fig:points}). In the range-based case, it may happen that a predicted anomaly range might partially overlap with a real one. In this case, a single prediction range is partially a TP and partially an FP at the same time. This introduces a gray area, which was not present in the point-based case. As in the classical model, the size of the partial overlap needs to be quantified, but there may be additional criteria. For example, we may also want to pay attention to the {\em position of the overlap}. After all, a range consists of an ordered collection of points and the order might be meaningful for the application. For instance, detecting the earlier portion of an anomaly (i.e., its "front-end" as illustrated in Figure \ref{fig:intervals}) might be more critical for a real-time application to reduce the time to react to it. Furthermore, overlaps are no longer 1-to-1 as in the classical model. One or more predicted anomaly ranges may (partially) overlap with one or more real anomaly ranges. Figure \ref{fig:intervals} illustrates one such situation. The application might care if each independent anomaly range is detected distinctly as a single unit or not. Thus, we may want to also capture so-called "{\em cardinality}" when measuring overlap. 

If all anomalies were point-based, or if there were no partial-overlap situations, then we could reuse the classical model, by simply treating each range in a sequence like a point in a set. In this case, size-based recall and precision measures would directly apply. For the more general case, a more expressive model that can evaluate partial overlaps is needed.

% TODO: We can mention this as part of Future Work, as our model currently does not capture these issues.
%In addition to partial overlaps, there can be other criteria due to the sequential nature of overlaps, such as relative anomaly size or distance (larger distance to a previous anomaly range representing a more rare occurrence). For example, an application might consider that missing a long/rare anomaly is worse than missing a short/frequent one.

Motivated by these observations, we would like to design a model that meets the following requirements:

\begin{itemize}
%[nosep,leftmargin=1em,labelwidth=*,align=left]
\item Expressive: Our model should be able to express criteria that are unique to range-based anomalies (e.g., size, position, and cardinality of partially overlapping ranges). Furthermore, since ranges are more general than points, our model should be able to subsume the classical point-based model.
\item Flexible: It should allow weighing multiple criteria in a tunable manner.
\item Extensible: One should be able to easily extend it with additional application-specific criteria as needed.
\end{itemize}

Intuitively, our model should enable ranking time-series AD algorithm results in a way that is as close to human judgment as possible.

\begin{comment}
\begin{verbatim}
Temporary notes:

Recall:
- Based purely on rewarding matches
- A weighted sum of value factors
  - Weights are adjustable
  - Value factors are extensible
- Base case: The only value factor is size.
- Corner cases:
  - No match gets 0 reward
  - All match gets 1 reward
  - All other cases are in-between
- If value factors and weights are adjusted properly, should be able
to rank results correctly.
- Example: TJ's current formula.

Precision:
- Based on penalizing mismatches?
\end{verbatim}
\end{comment}

==> related.tex <==
\section{Related Work} \label{sec:related}

There is a growing body of research emphasizing the importance of time-series anomaly detection. Bailis et al.'s work focuses on prioritization techniques when analyzing fast, streaming data including time-series outlier detection \cite{bailis:2017:macrobase}. Malhotra et al. and Guha et al. have proposed new ML techniques to handle time-series anomalies, ranging from space shuttles to Amazon web services~\cite{malhotra:2015:esann, guha:2016:icml}. Lipton et al. have investigated the viability of existing ML anomaly detection techniques on medical time-series data \cite{lipton:2015:iclr}, while Patcha and Park have drawn out weaknesses for anomaly detection systems to properly handle cyber-attacks in a time-series setting, among others~\cite{patcha:2007:survey}.

Despite  these advances, the measurement techniques applied to judge the efficacy of time-series anomaly detection systems are insufficient. They largely rely on classical recall and precision measurements, which have limitations when applied on range-based anomalies. This is a serious shortcoming in terms of guiding and refining the future generation of ML models and algorithms.
%largely based on classical definitions of recall and precision, which, as we argue throughout this paper, may be misrepresentative of not only the results, but can misguide the ML training techniques. This is because these same measurements of accuracy are used as feedback to guide and refine the generation of ML models.

We are not the first ones to make this observation. Lavin and Ahmad have also discussed the lack of proper time-series measurement techniques for anomaly detection in their Numenta Anomaly Benchmark (NAB) \cite{lavin:anomaly:2015}. Similar to our findings, they note the limitations of classical recall and precision in accurately measuring anomaly detection systems. Focusing specifically on real-time streaming applications, they state that: \emph{(i)} only early anomaly detection matters (i.e., front-end bias) and \emph{(ii)} only the first point of the anomaly range matters (i.e., an emphasis of precision over recall and a bias toward single-point positive prediction systems). They then continue to propose an anomaly scoring system based on anomaly windows, application profiles, and a sigmoidal scoring function, which is specifically designed to reward detections earlier in a window. 

While such a system may be suitable for their restricted domain, it is not generally applicable to range-based anomalies. For example, in some time-series scenarios such as the identification of medical anomalies (e.g., cancer detection), it is critical to capture when an illness is recessing due to the use of life threatening medical treatments used to address such illnesses~\cite{formenti:2017:cancer}. Under Lavin and Ahmad's single-point reward system there is no clear distinction for such state changes, because the single-point prediction algorithm and the scoring system that they propose only indicate the presence of an anomalous state, not the beginning or ending of it. Furthermore, as discussed in detail in a follow-up analysis by Singh and Olinsky \cite{singh-ijcnn17}, the NAB scoring system has a number of limitations that makes it hard to use in real-world applications, even within its restricted domain (e.g., the need to determine window size in advance, ambiguities in scoring function).

%For an anomaly detection measurement system to be used more generally, it must be expressive, flexible, and extensible (see Section \ref{sec:motivation}). 
Unlike Lavin and Ahmad's approach, our accuracy model does not have a fixed disposition to a single domain. Rather, it is general and flexible enough to support multiple application scenarios, including the classical recall/precision measures and Numenta's front-end bias scoring system, among potentially many others, as we demonstrate with experiments in Section \ref{sec:experiments}.
%In Section \ref{sec:experiment}, we present a detailed experimental study which demonstrates that our system not only subsumes the Numenta and the classical approaches, but significantly expands on them.

%0. Briefly mention that classical precision and recall are fundamentally rooted in point-based anomalies (Outlier analysis: https://dl.acm.org/citation.cfm?id=2436823). Fbeta scores allow for bias for one or another, which is a trade-off between precision and recall but doesn't include trade-offs for anomalous bias in time-series events.

%1. Emphasize the importance of time-series anomalies (self-driving cars level 4 and 5 are strictly anomaly detection and management robustness https://www.vtpi.org/avip.pdf) and their challenges (Google streaming anomaly detection dropouts: https://research.google.com/pubs/pub46283.html) 

%2. Discuss approaches to manage this space:

%a. LSTM-AD as a modeling system for anomalies over time and time series clustering ($https://link.springer.com/chapter/10.1007/978-3-642-02397-2_4$)
 
%b. Macrobase for emphasis on fast data streams and prioritization of attention for anomalies ($https://dl.acm.org/citation.cfm?id=3035918.3035928$)

%c. Amazon's real time anomaly detection, ICML 2016 (https://aws.amazon.com/kinesis/analytics/whitepaper-real-time-anomaly-detection/)
 
%3. Yet, no amount of modeling will provide reasonable solutions if the measurements of the accuracy of anomaly detection for time-series data is insufficient. As such, discuss the need to improve fundamentals:

%a. Numenta as an anomaly detection measurement for real-time anomalies. Yet it does not allow for flexible bias control for front-end or tail-end biases on anomaly detection.
 
%b. which leads us to this work



